ChatCoT: Tool-Augmented Chain-of-Thought Reasoning on Chat-based Large Language Models

Although large language models (LLMs) have achieved excellent performance in a variety of evaluation benchmarks, they still struggle in complex reasoning tasks which require specific knowledge and multi-hop reasoning. To improve the reasoning abilities, we propose ChatCoT, a tool-augmented chain-of-thought reasoning framework for chat-based LLMs (e.g., ChatGPT). In ChatCoT, we model the chain-of-thought (CoT) reasoning as multi-turn conversations, to utilize tools in a more natural way through chatting. At each turn, LLMs can either interact with tools or perform the reasoning. Our approach can effectively leverage the multi-turn conversation ability of chat-based LLMs, and integrate the thought chain following and tools manipulation in a unified way. Specially, we initialize the early turns of the conversation by the knowledge about tools, tasks, and reasoning format, and propose an iterative tool-augmented reasoning step to perform step-by-step tool-augmented reasoning. The experiment results on two complex reasoning datasets (MATH and HotpotQA) have shown the effectiveness of ChatCoT on complex reasoning tasks, achieving a 7.9% relative improvement over the state-of-the-art baseline. Our code and data are available at: \url{https://github.com/RUCAIBOX/ChatCoT}.

==> sections/approach_backup.tex <==
\section{Approach}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure/framework.pdf}
    \caption{The illustration of ChatCoT}
    \label{framework}
\end{figure*}

Multi-round dialogue is a natural way when human discuss with others to solve complex problem.
We utilize multi-round dialogue to help LLMs solve multi-hop reasoning problems.
In this section, we present \textbf{ChatCoT} which is a framework help LLMs to decompose problem and manipulate tools on complex reasoning tasks via multi-round dialogue.
Figure~\ref{framework} is an illustration of ChatCoT.

\subsection{Multi-step reasoning via multi-round dialogue}

The major advantage of multi-round dialogue is that it can convert a single reasoning process into several steps more natural than tradition CoT.
By leveraging the chatting ability of LLMs, we design an assistant based on rule which communicates with LLMs to guide LLMs reasoning step by step and help LLMs interact with external tools.

\subsubsection{Decomposing reasoning}

Classical CoT prompt strategy is used to guiding LLMs to generate analysis in natural language when solving reasoning tasks.
Formally, given the description of problem $D$ and prompt $P$, LLMs follow the example and instruction in $P$ to generate the solution $S=\{s_1, s_2, \dots, s_n\}$ of problem $D$, where $s_i=\{t_{i,1}, t_{i, 2}, \dots, t_{i, l_i}\}$ which is natural language denotes a single reasoning step of solution, and $t_{i,j}$ denotes the $j$-th token in the $i$-th reasoning step.

In ChatCot, each reasoning step can be view as one round of dialogue, and the full reasoning path $S$ can be transform into dialogue history $H$.
Through multi-round dialogue with rule based assistant, LLMs reason step by step and finally solve the problem.
For details, given a reasoning problem $D$, assistant will ask LLMs to decompose this problem and solve the sub-problem.
According to the problem and prompt, LLMs decompose the problem and generate corresponding reasoning step $s_i$.
Then, assistant utilize template to construct prompt to encourage LLMs to continue reasoning.
By analogy, LLMs decompose the complex problem into sub-problems and solve it step by step.
Figure~\ref{} is an example of problem decomposing and reasoning step by step in ChatCoT.

Formally, the full reasoning process can be represented by follow equations.
The speaker is on the left of colon, and the dialogue content is on the right of colon.
\begin{align}
\text{Assistant}&:~\texttt{Prompt}(D) \nonumber \\
\text{LLMs}&:~s_1 = \{t_{1,1}, t_{1, 2}, \dots, t_{1, l_1}\} \nonumber \\
\text{Assistant}&:~\texttt{Prompt}(s_1) \nonumber \\
\dots&:~\dots \nonumber \\
\text{LLMs}&: s_n = \{t_{n,1}, t_{n, 2}, \dots, t_{n, l_n}\},~A \nonumber
\end{align}
$\texttt{Prompt}(x)$ is a function to select template by rule based method and generate prompt according to the input $x$.
Given the description of problem $D$, assistant utilize function $\texttt{Prompt}(D)$ to obtain the prompt of problem and feed it into LLMs.
Then, LLMs generate reasoning steps and interact with assistant until reach the final answer.
Once reaching the final answer, LLMs will generate the answer $A$ in specific template, and assistant will extract the final answer from response of LLMs and finish dialogue process.

\begin{algorithm}
  \caption{Tool manipulation}\label{tool_manipulation}
\small
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{Sample}{Sample}\SetKwFunction{MaskMLM}{MaskMLM}\SetKwFunction{MaskDAE}{MaskDAE}
    \SetKwInOut{Input}{Input}\SetKwInOut{Parameter}{Parameter}
    \SetKwRepeat{Do}{do}{while}

    \Input{The history of dialogue $H$}
    \BlankLine
    Ask LLMs about which tools they need\;
    \If {LLMs do not need tools} {
        Encourage LLMs continue reasoning;\
    }
    \Else {
        \Do {Results are not useful} {
            Ask LLMs about parameters of tools\;
            Obtain the results of tools\;
            Ask LLMs whether the results are useful\;
        }
        Encourage LLMs continue reasoning;\
    }
\end{algorithm}

\subsubsection{Tool manipulation}

Complex reasoning problems usually require language models having specific knowledge (\eg mathematical knowledge, fine-grain commonsense knowledge) and various kinds of skills (\eg numerical computation, equation solving).
The utilization of external tools is an effective way to overcome the shortcomings of LLMs.
By utilizing multi-round dialogue for reasoning tasks, ChatCoT provide an effective way for LLMs to interact with external tools.
Algorithm~\ref{tool_manipulation} is the pesudo code of tool manipulation in ChatCoT.

\paratitle{Interaction with external tools}
At the beginning of reasoning, assistant provides LLMs with the information about the function and usage of external tools (\eg calculator, equation solver, retriever) and asks LLMs to utilize tools to reduce the mistakes, before giving the description of problem
During reasoning, assistant try to make query to LLMs about whether manipulating external tools and which tools should be chosen when LLMs generate one step of solution.
According to the query from assistant and the last reasoning steps, LLMs choose the corresponding tools (or not use tools) and generate the response to assistant.
Given the decision of LLMs, assistant either encourages LLMs continue reasoning when LLMs do not need the help of tools, or make query about the parameters of tools when LLMs have chosen the specific external tools.
If LLMs need the help of tools, they communicate with assistant to pass the parameters of tools and obtain the results from tools.

\paratitle{Feedback of results}
For several external tools, LLMs might not be satisfied with the results from these tools.
For example, in commonsense reasoning tasks, LLMs need some specific knowledge to solve the problem and ask assistant to use retriever to retrieve related corpus as evidence.
Obviously, retriever cannot always retrieve corpus that is helpful to LLMs.
In this case, LLMs have to send feedback to assistant and ask to retrieve corpus again in order to get useful information.
Therefore, the feedback of results from LLMs is necessary and is effective to improve the performance of LLMs on complex reasoning tasks.
In ChatCoT, with the help of multi-round dialogue, LLMs can communicate with assistant to send the feedback about the result of external tools, and assistant can follow the feedback to obtain the useful results from tools.

\subsection{Prompt construction for in-context learning}

In-context learning is an effective method to boost the performance of LLMs~\cite{}.
LLMs can learning task description and similar knowledge from the examplars in context.
For ChatCoT, we present the prompting strategy by mixing the retrieval examplars and annotated examplars in order to provide useful knowledge and instruct LLMs to reason through multi-round dialogue.

\paratitle{Retrieve similar examplars}
In knowledge-intensive reasoning tasks, LLMs cannot perform well because of lack of domain specific knowledge which is necessary to solve the problem.
For example, in mathematical problem, LLMs can learn related knowledge and reasoning methods from similar problems.
Providing similar problem as examplars for LLMs can significantly improve the performance of LLMs in knowledge-intensive reasoning tasks.
Thus, in ChatCoT, we utilize SimCSE~\cite{} to retrieve the similar problem as examplars in prompt.
First, we have trained SimCSE on the connection of problem and solution in training set via unsupervised training methods in order to teach retriever to the meaning of special tokens (\eg latex tokens in mathematical problem) and adapt to the specific domain.
Second, we leveragy a well-trained SimCSE model as the retriever to retrieval similar problems.
For a test problem, we retrieve $n_r$ similar problems from training set as examplars for LLMs.

\paratitle{Annotated chatting form examplars}
In order to induce LLMs reasoning through multi-round dialogue, manual annotated examplars are necessary.
We randomly select $5$ problems from full training set which includes all sub-tasks in the benchmark as the candidate set.
The selected problems have been annotated in multi-round dialogue form where LLMs reason step by step and communicate with assistant about the usage of external tools.
Specially, these annotated chatting form examplars will be feed into LLMs through dialogue history instead of a paragraph of natural language.
In this way, LLMs can follow the examplars and reason through multi-round dialogue better.
In practice, we randomly choose $n_a (n_a \leq 5)$ problems from candidates set as examplars.

In order to better mix these two type examplars, we conduct the examplars via dialogue format.
The retrieval examplars will be connected into a paragraph $P_r = \{D_1, A_1, \dots, D_{n_r}, A_{n_r}\}$ and assistant inform LLMs that $P_r$ contains useful knowledge which can be used in inference.
In other words, the retrieval examplars can be conduct in a single round dialogue.
Together with Annotated examplars, these two kinds of exampalrs will be feed into LLMs via dialogue history.
The number of exmplars in prompt is $n_r + n_a$.

\subsection{Augment modules adaption}

Although ChatCoT guide LLMs reasoning step by step through multi-round dialogue which is different from classical CoT, ChatCoT can also adapt to the augment modules which are designed for CoT, such as self-consistency and self-refine.
% Decomposition Enhances Reasoning via Self-Evaluation Guided Decoding
Besides, with decomposing reasoning, the methods about decoding strategy~\cite{} can also be used in ChatCoT to boost the performance.
In this section, we introduce the methods to adapt ChatCoT to augment modules, and take self-consistency and self-refine as representative works.

\paratitle{Consistency}
The main idea of self-consistency is generating diversified reasoning path to get several answers and selecting the most confident answer through voting.
Formally, the score the each answer can be calculated by follow equation, and the answer getting the highest score will be chosen as the final answer.
$$
\text{Score}(A_i) = \sum_{p=1}^{k}{\mathbbm{1}[A_p == A_i]}
$$
Where $k$ denotes the number to generated reasoning path, and $A_i$ is the answer of $i$-th reasoning path.
ChatCoT can also generate diversified multi-round dialogue which has similar function with reasoning path in CoT via adjusting the temperature parameters.
By leveraging diversified multi-round dialogue, ChatCoT can obtain several answers and get the final answer by ensemble.
Empirical study shows that ChatCoT adapts to self-consistency better than classical CoT method.

\paratitle{Refinement}
For refinement, a convenient method is converting mulit-round dialogue into a paragraph of reasoning in natural language.
First, to convert dialogue history into a paragraph of natural language, the prompt and instruction which guide LLMs to decompsing reasoning and manipulating external tools is not necessary.
Therefore, we delete these content containing useless information and keep the content including reasoning steps and results from external tools.
By connecting the remaining content together without the name of speaker, the reasoning path in natural language will be obtained and can be used in refinement.
By converting multi-round dialogue into reasoning path in natural language, it can easily adapt to the refinement methods like self-refine.
